On the Benefit of Adversarial Training for Monocular Depth Estimation

In this paper we address the benefit of adding adversarial training to the task of monocular depth estimation. A model can be trained in a self-supervised setting on stereo pairs of images, where depth (disparities) are an intermediate result in a right-to-left image reconstruction pipeline. For the quality of the image reconstruction and disparity prediction, a combination of different losses is used, including L1 image reconstruction losses and left-right disparity smoothness. These are local pixel-wise losses, while depth prediction requires global consistency. Therefore, we extend the self-supervised network to become a Generative Adversarial Network (GAN), by including a discriminator which should tell apart reconstructed (fake) images from real images. We evaluate Vanilla GANs, LSGANs and Wasserstein GANs in combination with different pixel-wise reconstruction losses. Based on extensive experimental evaluation, we conclude that adversarial training is beneficial if and only if the reconstruction loss is not too constrained. Even though adversarial training seems promising because it promotes global consistency, non-adversarial training outperforms (or is on par with) any method trained with a GAN when a constrained reconstruction loss is used in combination with batch normalisation. Based on the insights of our experimental evaluation we obtain state-of-the art monocular depth estimation results by using batch normalisation and different output scales.

==> tables/ablation_study.tex <==
\begin{table*}[t]
    \centering
    \caption{Ablation study of loss components. All parameters $\gamma$ weigh loss components from equation \ref{eq:single_scale_loss_plus_occlusion}. $\alpha_{\text{SSIM}}$ is the ratio between L1 and SSIM.}
    \resizebox{1.0\textwidth}{!}{
        \begin{tabular}{@{\extracolsep{4pt}}ccccc||ccccccc@{}}
        \hline
        \multicolumn{5}{c|}{Loss Weights $\gamma$} & ARD & SRD & RMSE  & RMSE log & $\delta < 1.25$ & $\delta < 1.25^{2}$ & $\delta < 1.25^{3}$ \\ 
        \cline{6-9} \cline{10-12}
        $\gamma_{l1}$ & $\gamma_{s}$ & $\gamma_{lr}$ & $\gamma_{disp}$ & $\gamma_{occl}$ & \multicolumn{4}{c}{lower is better} & \multicolumn{3}{c}{higher is better} \\ \hline
        1.0 & 0.0 & 0.0 & 0.0 & 0.0                     & 0.212 & 3.628 & 7.271 & 0.308 & 0.747 & 0.893 & 0.949 \\
        0.5 & 0.5 & 0.0 & 0.0 & 0.0                     & 0.143 & 1.199 & 5.709 & 0.239 & 0.808 & 0.927 & \cellcolor{LightCyan} \textbf{0.968} \\
        0.15 & 0.85 & 0.0 & 0.0 & 0.0                   & \cellcolor{LightCyan} \textbf{0.142} & \cellcolor{LightCyan} \textbf{1.186} & 5.689 & 0.238 & 0.808 & 0.927 & \cellcolor{LightCyan} \textbf{0.968} \\
        0.0 & 1.0 & 0.0 & 0.0 & 0.0                     & \cellcolor{LightCyan}\textbf{0.142} & 1.197 & \cellcolor{LightCyan} \textbf{5.637} & \cellcolor{LightCyan} \textbf{0.237} & \cellcolor{LightCyan} \textbf{0.811} & \cellcolor{LightCyan} \textbf{0.928} & \cellcolor{LightCyan} \textbf{0.968} \\
        & & & & & & & & & & & \\
        0.0 & 0.0 & 1.0 & 0.0 & 0.0                     & 1.000 & 16.087 & 19.776 & 9.500 & 0.0 & 0.0 & 0.0 \\
        1.0 & 0.0 & 1.0 & 0.0 & 0.0                     & 0.200 & 3.187 & 6.898 & 0.292 & 0.759 & 0.902 & 0.954 \\
        0.15 & 0.85 & 1.0 & 0.0 & 0.0                   & \cellcolor{LightCyan} 0.144 & \cellcolor{LightCyan} 1.215 & \cellcolor{LightCyan} 5.688 & \cellcolor{LightCyan} 0.240 & \cellcolor{LightCyan} 0.807 & \cellcolor{LightCyan} 0.926 & \cellcolor{LightCyan} 0.967 \\
        & & & & & & & & & & & \\
        0.15 & 0.85 & 1.0 & 0.1 & 0.0                   & \cellcolor{LightCyan} \textbf{0.142} & \cellcolor{LightCyan} 1.200 & \cellcolor{LightCyan} 5.694 & \cellcolor{LightCyan} 0.239 & \cellcolor{LightCyan} 0.809  & \cellcolor{LightCyan} 0.927 & \cellcolor{LightCyan} 0.967 \\
        0.15 & 0.85 & 1.0 & 0.0 & 0.01                  & 0.143 & 1.209 & 5.730 & 0.241 & 0.805 & \cellcolor{LightCyan} 0.927 & \cellcolor{LightCyan} 0.967 \\
        0.15 & 0.85 & 1.0 & 0.1 & 0.01                  & \cellcolor{LightCyan} \textbf{0.142} & 1.202 & 5.706 & 0.240 & 0.807 & \cellcolor{LightCyan} 0.927 & \cellcolor{LightCyan} 0.967 \\
        0.15 & 0.85 & 1.0 & 0.25 & 0.25                 & 0.190 & 4.000 & 6.905 & 0.278 & 0.798 & 0.918 & 0.960 \\
        0.15 & 0.85 & 1.0 & 1.0 & 1.0                   & 0.625 & 32.436 & 14.880 & 0.517 & 0.733 & 0.847 & 0.892 \\
        \hline
        \end{tabular}
    }
    \label{tab:ablation_study_loss_components}
\end{table*}


==> tables/comparison_extended.tex <==
\begin{table*}[t]
    \centering
    \caption{Comparison of RN50 architecture with method of \citet{godard2017unsupervised}, when pre-trained on CityScape (SC) dataset.}
    \resizebox{1\textwidth}{!}{
        \begin{tabular}{@{\extracolsep{4pt}}lcc||ccccccc@{}}
        \hline
        \multirow{2}{*}{Method}  & \multirow{2}{*}{} & \multirow{2}{*}{Trained on}
        & ARD & SRD & RMSE & RMSE log & $\delta < 1.25$ & $\delta < 1.25^{2}$ & $\delta < 1.25^{3}$ \\ 
        \cline{4-7} \cline{8-10}
        & & & \multicolumn{4}{c}{lower is better} & \multicolumn{3}{c}{higher is better} \\
        \hline
        \multicolumn{3}{l||}{\bf Supervised using Left-Right Correspondence} & & \\                   
        \citet{pilzer2018unsupervised} &  & K  & 0.152 & 1.388 & 6.016 & 0.247 & 0.789 & 0.918 & 0.965 \\
        \citet{godard2017unsupervised} & VGG & K   & 0.148 & 1.344 & 5.927 & 0.247 & 0.803 & 0.922 & 0.964 \\
        \bf Our work & baseline & K                           & 0.142 & 1.200 & 5.694 & 0.239 & 0.809 & 0.927 & 0.967 \\
        \bf Our work & BN + S2 & K &  \textbf{0.128} & \bf 1.026 & \bf 5.313 & \textbf{0.222} & \textbf{0.830} & \textbf{0.939} & \bf 0.973 \\
        \hline
        \citet{godard2017unsupervised} & RN50 & CS + K               & 0.114 & 0.898 & 4.935 & 0.206 & 0.861 & 0.949 & 0.976 \\
        \bf Our work & RN50+BN+S2 & CS + K                & \bf 0.112 & \bf 0.820 & \bf 4.738 &\bf  0.202 & \bf 0.866 & \bf 0.952 & \bf 0.978 \\
        \hline        
        \end{tabular}
    }
    
    \label{tab:other_methods_comparison}
\end{table*}

==> tables/overview.tex <==
% !TEX root =  depthgan19cviu.tex
\begin{table*}[p]
	\centering
	\caption{Performance of models using different GAN variants. Cropping from \citet{garg2016unsupervised} was used for evaluation. For all results post-processing of disparity maps was performed.}
	\resizebox{0.95\textwidth}{!}{
		\begin{tabular}{lc@{\hspace{1mm}}c@{\hspace{1mm}}c@{\hspace{1mm}}c@{\hspace{1mm}}c|@{\hspace{1mm}}c@{\hspace{1mm}}|@{\hspace{1mm}}c@{\hspace{1mm}}||ccccccc@{}}
			\hline
			&\multicolumn{5}{c}{Loss Components} & \multirow{2}{*}{BN} & \multirow{2}{*}{GAN} & ARD & SRD & RMSE  & RMSE log & $\delta\!<\!1.25$ & $\delta\!<\!1.25^{2}$ & $\delta\!<\!1.25^{3}$ \\ 
			\cline{9-12} \cline{13-15}
			& L1 & LR & Disp & Occl & SSIM & & & \multicolumn{4}{c}{lower is better} & \multicolumn{3}{c}{higher is better} \\ 
			\hline			
			1 & & & & & & \checkmark & V                        &\cellcolor{LightCyan} 0.810 & 12.442 & 18.245 & 1.999 &\cellcolor{LightCyan} 0.002 & \cellcolor{LightCyan} 0.008 &\cellcolor{LightCyan} 0.020 \\
			1 & & & & & & \checkmark & LS                          & 0.893 & 13.826 & 18.816 & 2.468 & 0.000 & 0.000 & 0.000 \\
			1 & & & & & & & W                                      & 0.813 &\cellcolor{LightCyan} 12.310 & \cellcolor{LightCyan}18.119 &\cellcolor{LightCyan} 1.932 & 0.001 & 0.003 & 0.011 \\
			& & & & & & & & & & & & & & \\
			
			2 & \checkmark & & & & & &                                & 0.215 & 3.685 & 7.302 & 0.307 & 0.746 & 0.894 & 0.949 \\
			2 & \checkmark & & & & & \checkmark &                     & 0.200 & 3.149 & 6.795 & 0.289 & 0.760 & 0.904 & 0.956 \\
			2 & \checkmark & & & & & \checkmark &  V            & 0.205 & 3.781 & 7.045 & 0.288 & \cellcolor{LightCyan}0.771 & \cellcolor{LightCyan}0.911 & 0.958 \\
			2 & \checkmark & & & & & \checkmark & LS               & 0.190 & 2.826 & 6.612 & 0.281 & 0.766 & 0.909 & \cellcolor{LightCyan}0.959 \\
			2 & \checkmark & & & & & & W                           &\cellcolor{LightCyan} 0.177 & \cellcolor{LightCyan}2.398 & \cellcolor{LightCyan}6.504 &\cellcolor{LightCyan} 0.275 & 0.770 & 0.905 & 0.957 \\
			& & & & & & & & & & & & & & \\			
			3 & \checkmark & \checkmark & & & & &                     & 0.191 & 2.661 & 6.710 & 0.285 & 0.760 & 0.904 & 0.956 \\
			3 & \checkmark & \checkmark & & & & \checkmark &          & 0.162 & 1.755 & \cellcolor{LightCyan}5.954 &\cellcolor{LightCyan} 0.253 & 0.789 & 0.922 &\cellcolor{LightCyan} 0.966 \\
			3 & \checkmark & \checkmark & & & & \checkmark & V  & 0.168 & 2.090 & 6.104 & 0.261 & 0.784 & 0.919 & 0.964 \\
			3 & \checkmark & \checkmark & & & & \checkmark & LS    & \cellcolor{LightCyan}0.160 & 1.761 & 5.966 &\cellcolor{LightCyan} 0.253 & \cellcolor{LightCyan}0.792 & \cellcolor{LightCyan}0.923 & \cellcolor{LightCyan}0.966 \\
			3 & \checkmark & \checkmark & & & & & W                & 0.170 & \cellcolor{LightCyan}1.521 & 6.121 & 0.258 & 0.769 & 0.909 & 0.960 \\
			& & & & & & & & & & & & & & \\
			
			4 & \checkmark & \checkmark & \checkmark & & & &                     & 0.200 & 3.155 & 7.039 & 0.295 & 0.758 & 0.900 & 0.953 \\
			4 & \checkmark & \checkmark & \checkmark & & & \checkmark &          & 0.163 & 1.842 & 5.978 & 0.253 & 0.791 & 0.922 & \cellcolor{LightCyan}0.966 \\
			4 & \checkmark & \checkmark & \checkmark & & & \checkmark & V  & 0.165 & 1.907 & 6.094 & 0.258 & 0.787 & 0.920 & 0.964 \\
			4 & \checkmark & \checkmark & \checkmark & & & \checkmark & LS    & \cellcolor{LightCyan}0.158 & 1.632 & \cellcolor{LightCyan}5.784 & \cellcolor{LightCyan} 0.248 &\cellcolor{LightCyan} 0.799 & \cellcolor{LightCyan}0.925 & \cellcolor{LightCyan}0.966 \\
			4 & \checkmark & \checkmark & \checkmark & & & & W                & 0.160 & \cellcolor{LightCyan}1.427 & 6.179 & 0.259 & 0.772 & 0.908 & 0.959 \\
			& & & & & & & & & & & & & & \\			
			5 & \checkmark & \checkmark & \checkmark & \checkmark & & &                     & 0.204 & 3.399 & 6.983 & 0.295 & 0.760 & 0.901 & 0.953 \\
			5 & \checkmark & \checkmark & \checkmark & \checkmark & & \checkmark &          & 0.165 & 1.955 & \cellcolor{LightCyan}6.028 & \cellcolor{LightCyan}0.256 &\cellcolor{LightCyan} 0.790 & \cellcolor{LightCyan}0.922 & \cellcolor{LightCyan}0.966 \\
			5 & \checkmark & \checkmark & \checkmark & \checkmark & & \checkmark & V  & 0.196 & 3.182 & 6.582 & 0.282 & 0.778 & 0.911 & 0.957 \\
			5 & \checkmark & \checkmark & \checkmark & \checkmark & & \checkmark & LS    & 0.174 & 2.236 & 6.137 & 0.263 & 0.785 & 0.917 & 0.962 \\
			5 & \checkmark & \checkmark & \checkmark & \checkmark & & & W                & \cellcolor{LightCyan}0.161 & \cellcolor{LightCyan}1.557 & 6.191 & 0.260 & 0.776 & 0.910 & 0.960 \\			
			& & & & & & & & & & & & & & \\
			6 & \checkmark & \checkmark & \checkmark & & \checkmark & &                       & 0.142 & 1.200 & 5.694 & 0.239 & 0.809 & 0.927 & 0.967 \\
			6 & \checkmark & \checkmark & \checkmark & & \checkmark & \checkmark & -          & \cellcolor{LightCyan}\textbf{0.132} & \cellcolor{LightCyan}1.049 & \cellcolor{LightCyan} {5.376} & \cellcolor{LightCyan}\textbf{0.224} & \cellcolor{LightCyan}\textbf{0.822} & \cellcolor{LightCyan}0.937 & \cellcolor{LightCyan}\textbf{0.974} \\
			6 & \checkmark & \checkmark & \checkmark & & \checkmark & \checkmark & V    & 0.135 & 1.052 & 5.428 & 0.229 & 0.818 & 0.935 & 0.972 \\
			6 & \checkmark & \checkmark & \checkmark & & \checkmark & \checkmark & LS      & 0.135 & 1.051 & 5.417 & 0.227 & 0.819 & 0.936 & 0.972 \\
			6 & \checkmark & \checkmark & \checkmark & & \checkmark & & W                  & 0.152 & 1.357 & 6.003 & 0.249 & 0.788 & 0.917 & 0.963 \\			
			& & & & & & & & & & & & & & \\
			7 & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & &                     & 0.142 & 1.205 & 5.726 & 0.240 & 0.806 & 0.927 & 0.967 \\
			7 & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark &          &\cellcolor{LightCyan}\bf 0.132 &\cellcolor{LightCyan}\bf 1.035 &\cellcolor{LightCyan}\bf 5.370 &\cellcolor{LightCyan}0.225 &\cellcolor{LightCyan}\bf 0.822 & 0.937 & \cellcolor{LightCyan}0.973 \\
			7 & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & V  & 0.133 & 1.055 & 5.390 &\cellcolor{LightCyan}0.225 &\cellcolor{LightCyan}\bf 0.822 &\cellcolor{LightCyan}\textbf{0.938}&\cellcolor{LightCyan}0.973 \\
			7 & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & LS    & 0.134 & 1.090 & 5.447 & 0.226 & 0.820 & 0.937 &\cellcolor{LightCyan}0.973 \\
			7 & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & & W                & 0.157 & 1.368 & 6.065 & 0.253 & 0.779 & 0.915 & 0.963 \\
			 & & & & & & & & & & & & & & \\
			\hline
			8 & \multicolumn{7}{c||}{\textbf{Training set mean}}                                    & 0.361 & 4.826 & 8.102 & 0.377 & 0.638 & 0.804 & 0.894 \\
			\hline
		\end{tabular}
	}
	\label{tab:overview_ext}
\end{table*}
